Regret Lower Bounds for Learning Linear Quadratic Gaussian Systems

TWe establish regret lower bounds for adaptively controlling an unknown linear Gaussian system with quadratic costs. We combine ideas from experiment design, estimation theory and a perturbation bound of certain information matrices to derive regret lower bounds exhibiting scaling on the order of magnitude $\sqrt{T}$ in the time horizon $T$. Our bounds accurately capture the role of control-theoretic parameters and we are able to show that systems that are hard to control are also hard to learn to control; when instantiated to state feedback systems we recover the dimensional dependency of earlier work but with improved scaling with system-theoretic constants such as system costs and Gramians. Furthermore, we extend our results to a class of partially observed systems and demonstrate that systems with poor observability structure also are hard to learn to control.

==> jour.tex <==

\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}



%%%%%%
%author may change 

\usepackage{authblk}
\author[1]{Ingvar Ziemann}
\author[2]{Henrik Sandberg}
\affil[1]{University of Pennsylvania}
\affil[2]{KTH Royal Institute of Technology}



%%%%%%


%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage[dvipsnames]{xcolor}

\usepackage{natbib}
\usepackage{enumitem}
%
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{hyperref}
\hypersetup{
 %   bookmarks=true,         % show bookmarks bar?
         % non-Latin characters in Acrobat’s bookmarks
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdfnewwindow=true,      % links in new PDF window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=blue,          % color of internal links (change box color with linkbordercolor)
    citecolor=ForestGreen,        % color of links to bibliography
    filecolor=magenta,      % color of file links
    urlcolor=red,           % color of external links
    breaklinks=false,
}

\usepackage{cleveref}
\usepackage{thmtools}
\usepackage{thm-restate}



==> sections/proofs.tex <==



\subsection{Proof of \Cref{thm:sfregretlb}}
Throughout the proof we use $\e= T^{-\alpha}$ and set $T$ sufficiently large such that the quantities $P(\cdot)$ and $K(\cdot)$ are continuous over $B(\theta,\e)$, which is guaranteed by our burn-in condition \cref{eq:burninsfregretlb} combined with Proposition 1 of \cite{mania2019certainty}. Moreover, we may assume that $ \sup_{\theta' \in B(\theta,\e)}\mathsf{R}_T^\pi(\theta) \leq C \sqrt{T}$ for a constant $C>0$ to be determined later. Before we proceed with the main argument of the proof, we also choose the matrix $W_0$ by defining its columns to be the eigenvectors corresponding to the $d$ smallest nonzero eigenvalues of $V_0^\T (\E \I (\Theta,\pi,T)+\J(\lambda))V_0$. This choice in particular yields that:
\begin{equation}
\label{eq:fishermanipul}
    \begin{aligned}
&\lambda_1 \left(W_0^\T (\E \I(\Theta,\pi,T)+\J(\lambda) )W_0\right)\\
    &\leq\lambda_{1+\dim \mathtt{U}-d} \left(V_0^\T (\E \I(\Theta,\pi,T)+\J(\lambda) )V_0\right)\\
    &\leq \frac{1}{1+\dim \mathtt{U}-d}\tr \left(V_0^\T (\E \I(\Theta,\pi,T)+\J(\lambda) )V_0\right)\\
    &\leq \frac{L R_{T}^\pi(\theta)+\tr(\J(\lambda))}{1+\dim \mathtt{U}-d}\\
    &\leq \frac{L C \sqrt{T}+\tr(\J(\lambda))}{1+\dim \mathtt{U}-d}.
    \end{aligned}
\end{equation}




The proof now proceeds by invoking \Cref{lem:regretlbrelaxed} and \eqref{eq:regretlbrelaxedSF} to relax the supremum in the theorem statement to an expectation, and in particular to find that:
\begin{align*}
  &\inf_\pi \sup_{\theta' \in B(\theta,\e)}\mathsf{R}_T^\pi(\theta)\\
    &\geq\sum_{t=0}^{T-1} \E_{\Theta \sim \lambda}\E_{\Theta}^\pi \tr \Big[N_\star  \left( \E[K(\Theta)|\mathcal{Y}_{T-1}]-K(\Theta)\right) \left(X_tX_t^\T \right) \left( \E[K(\Theta)|\mathcal{Y}_{T-1}]-K(\Theta) \right)^\T \Big].
\end{align*}
Introduce further a positive semi-definite matrix $\Psi$ and the event 
\begin{align*}
    \mathcal{E}\triangleq \left\{ \sum_{t=0}^{T-1} X_tX_t^\T \succeq \Psi T \right\}.
\end{align*}
By definition of $\mathcal{E}$:
\begin{equation}
\begin{aligned}
\label{eq:calcinsfproof_1}
   & \inf_\pi \sup_{\theta' \in B(\theta,\e)}\mathsf{R}_T^\pi(\theta)\\
    &\geq\sum_{t=0}^{T-1} \E_{\Theta \sim \lambda}\E_{\Theta}^\pi \tr \Big[N_\star  \left( \E[K(\Theta)|\mathcal{Y}_{T-1}]-K(\Theta)\right) \left(X_tX_t^\T \right) \left( \E[K(\Theta)|\mathcal{Y}_{T-1}]-K(\Theta) \right)^\T \Big]\\
    &\geq \E_{\Theta \sim \lambda}\E_{\Theta}^\pi \tr \Big[N_\star  \left( \E[K(\Theta)|\mathcal{Y}_{T-1}]-K(\Theta)\right) \left( \sum_{t=0}^{T-1} X_tX_t^\T \right) \left( \E[K(\Theta)|\mathcal{Y}_{T-1}]-K(\Theta) \right)^\T \Big]\\
    &\geq T \E_{\Theta \sim \lambda}\E_{\Theta}^\pi \tr \Big[N_\star  \left( \E[K(\Theta)|\mathcal{Y}_{T-1}]-K(\Theta)\right) \mathbf{1}_{\mathcal{E}} \Psi \left( \E[K(\Theta)|\mathcal{Y}_{T-1}]-K(\Theta) \right)^\T \Big]\\
    &\geq T \E_{\Theta \sim \lambda}\E_{\Theta}^\pi  \left\| \VEC  \left( \E[\sqrt{N_\star}K(\Theta)\sqrt{\Psi}|\mathcal{Y}_{T-1}]-\sqrt{N_\star}K(\Theta)\sqrt{\Psi}\right) \mathbf{1}_{\mathcal{E}} \right\|_2^2.
\end{aligned}
\end{equation}
We now continue by writing the norm (inner product) in \eqref{eq:calcinsfproof_1} as the trace of an outer product:
\begin{equation}
\begin{aligned}
   \eqref{eq:calcinsfproof_1}  &= T \tr \Bigg( \VEC \left( \E[\sqrt{N_\star}K(\Theta)\sqrt{\Psi}|\mathcal{Y}_{T-1}]-\sqrt{N_\star}K(\Theta)\sqrt{\Psi}\right)\\
    &\times \VEC \left( \E[\sqrt{N_\star}K(\Theta)\sqrt{\Psi}|\mathcal{Y}_{T-1}]-\sqrt{N_\star}K(\Theta)\sqrt{\Psi}\right)^\T  \mathbf{1}_{\mathcal{E}}\Bigg)\\
    &= \tr \left( (\Psi \otimes N_\star) \left(\VEC \left(\E[K(\Theta)|\mathcal{Y}_{T-1}]-\VEC K(\Theta) \right)\left(\E[K(\Theta)|\mathcal{Y}_{T-1}]-\VEC K(\Theta) \right)^\T  \right) \right).
\end{aligned}
\end{equation}
Since $\E[K(\Theta)|\mathcal{Y}_{T-1}]$ is an estimator of $K(\Theta)$, we may apply \Cref{thm:vtineq} combined with monotonicity of the trace in semidefinite order to find:
\begin{equation}
\label{eq:calc:in:sfproof}
    \begin{aligned}
 &T \tr \left( (\Psi \otimes N_\star) \left(\VEC \left(\E[K(\Theta)|\mathcal{Y}_{T-1}]-\VEC K(\Theta) \right)\left(\E[K(\Theta)|\mathcal{Y}_{T-1}]-\VEC K(\Theta) \right)^\T  \right) \right)\\
 %%
 &\geq T \tr \left((\Psi \otimes N_\star)  (\dop_\theta K(\Theta) W_0) \left( W_0^\T\E \I(\Theta,\pi,T)W_0+W_0^\T\J(\lambda)W_0 \right)^{-1} W_0^\T ( \dop_\theta K(\Theta))^\T   \right)     
    \end{aligned}
\end{equation}

Hence, if we combine \eqref{eq:calc:in:sfproof} with \eqref{eq:fishermanipul} we find that:
\begin{equation}
    \begin{aligned}\label{eq:fisherisbddinsfproof}
    &\inf_\pi \sup_{\theta' \in B(\theta,\e)}\mathsf{R}_T^\pi(\theta)\\
    &\geq  \frac{T(1+\dim \mathtt{U}-d)}{L C \sqrt{T}+\tr(\J(\lambda))}   \mathbf{P}^2(\mathcal{E}) \inf_{\theta',\tilde\theta \in B(\theta,\e)}\tr \Bigg((\Psi\otimes N_\star)(\dop_\theta \VEC(K(\theta'))\\
&\times W_0W_0^\T (\dop_\theta \VEC(K(\theta'))^\T\Bigg).
    \end{aligned}
\end{equation}
We will show that if  for some (universal) polynomial function $\mathsf{poly}$
\begin{align}\label{eq:omitteddisplay}
    T\geq \sup_{\theta'\in B(\theta,\e)}\mathsf{poly}\left(9^{\dx},\opnorm{B},\opnorm{A},\opnorm{Q^{-1}}\opnorm{R},\opnorm{R^{-1}},\opnorm{B},\opnorm{P},\opnorm{K},\opnorm{\Sigma_W},C \right)
\end{align}
where we have omitted dependency on $\theta'$ in the arguments of $\mathsf{poly}$ in \eqref{eq:omitteddisplay}. We show that $\mathbf{P}(\mathcal{E})\geq 1/2$ with any $\Psi$  satisfying
\begin{align*}
    \Psi \preceq\sum_{j=0}^{T^{1/16}}(A(\theta')+B(\theta')K(\theta'))^j\Bigg[ \Sigma_W  -I_{\dx}(\opnorm{\Sigma_W}T^{-1/4}+T^{-1/4}+T^{-1/8})\Bigg]((A(\theta')+B(\theta')K(\theta'))^\T)^j 
\end{align*}
 for all $\theta' \in B(\theta,\e)$ in \Cref{sec:boundPEN}. Taking this for granted for now, we now choose
\begin{align*}
    C =   \sqrt{\frac{(1+\dim \mathtt{U}-d)}{ 8 L  }}\sqrt{ \inf_{\theta',\tilde\theta \in B(\theta,\e)}\tr \Bigg((\Psi\otimes N_\star)(\dop_\theta \VEC(K(\theta'))
 W_0W_0^\T (\dop_\theta \VEC(K(\theta'))^\T\Bigg)}.
\end{align*}
Hence with this choice of $C$ and as long as $\sqrt{T} \geq\frac{\tr\J(\lambda)}{LC}$ we are guaranteed that 
\begin{equation}
    \begin{aligned}\label{eq:fisherisbddinsfproof3}
    &\inf_\pi \sup_{\theta' \in B(\theta,\e)}\mathsf{R}_T^\pi(\theta)\\
    &\geq  \sqrt{T} \sqrt{\frac{1+\dim \mathtt{U}-d}{8L}}\sqrt{ \inf_{\theta',\tilde\theta \in B(\theta,\e)}\tr \Bigg((\Psi\otimes N_\star)(\dop_\theta \VEC(K(\theta'))
 W_0W_0^\T (\dop_\theta \VEC(K(\theta'))^\T\Bigg)}.
    \end{aligned}
\end{equation}
This finishes the proof, since if $\sup_{\theta' \in B(\theta,\e)}\mathsf{R}_T^\pi(\theta) \leq C\sqrt{T}$ does not hold for our choice of $C$, \eqref{eq:fisherisbddinsfproof3} holds trivially. \hfill $\blacksquare$

\subsubsection{Bounding $\mathbf{P}(\mathcal{E})$}
\label{sec:boundPEN}

Fix any $\theta' \in B(\theta,\e)$ and denote $A=A(\theta'),B=B(\theta')$, $P=P(\theta')$, $\mathsf{R}_T^\pi=\mathsf{R}_T^\pi(\theta')$ and $K=K(\theta')$ to avoid cumbersome notation.\footnote{This convention applies to \Cref{sec:boundPEN} alone.} The evolution of $X_tX_t^\T$ under $\theta'$ is given by:
\begin{equation}
\begin{aligned}\label{eq:xtxttopequation}
    X_tX_t^\T &= (AX_{t-1}+BU_{t-1}+W_{t-1})(AX_{t-1}+BU_{t-1}+W_{t-1})^\T\\
              &= ((A+BK)X_{t-1}+B(U_{t-1}-KX_{t-1})+W_{t-1})\\
              &\times((A+BK)X_{t-1}+B(U_{t-1}-KX_{t-1})+W_{t-1})^\T\\
              &=(A+BK)X_{t-1}X_{t-1}^\T(A+BK)^\T\\
              &+(B(U_{t-1}-KX_{t-1})+W_{t-1})(B(U_{t-1}-KX_{t-1})+W_{t-1})^\T \\
              &+\sym (A+BK)X_{t-1}(B(U_{t-1}-KX_{t-1})+W_{t-1})^\T\\
              &\succeq (A+BK)X_{t-1}X_{t-1}^\T(A+BK)^\T+W_{t-1}W_{t-1}^\T\\
              &+\sym B(U_{t-1}-KX_{t-1}))(W_{t-1})^\T \\
              &+\sym (A+BK)X_{t-1}(B(U_{t-1}-KX_{t-1})+W_{t-1})^\T \\
              &=(A+BK)X_{t-1}X_{t-1}^\T(A+BK)^\T+W_{t-1}W_{t-1}^\T\\
              &+\sym\left[ B(U_{t-1}+AX_{t-1}))\right](W_{t-1})^\T \\
              &+\sym (A+BK)X_{t-1}(B(U_{t-1}-KX_{t-1}))^\T
\end{aligned}
\end{equation}
where $\sym M = M+M^\T$ for any matrix $M$. If we iterate \eqref{eq:xtxttopequation} $m$ times, sum over $t$ and exchange the order of summation we obtain:
\begin{equation}
\begin{aligned}\label{eq:xtxttopequation2}
   \sum_{t=0}^{T-1} X_tX_t^\T &=\sum_{j=0}^{m}(A+BK)^j\Bigg[\sum_{t=0}^{T-1}W_{t-j}W_{t-j}^\T\Bigg]((A+BK)^\T)^j\\
              &+\sum_{j=0}^{m}(A+BK)^j\Bigg[\sum_{t=0}^{T-1}\sym\left[ B(U_{t-j}+AX_{t-j}))\right](W_{t-j})^\T\Bigg]((A+BK)^\T)^j \\
              &+\sum_{j=0}^{m}(A+BK)^j\Bigg[\sum_{t=0}^{T-1}\sym (A+BK)X_{t-j}(B(U_{t-j}-KX_{t-j}))^\T\Bigg]((A+BK)^\T)^j.
\end{aligned}
\end{equation}
where quantities with negative indices are taken to be zero.

The strategy is now as follows. We wish to show that the first term in \eqref{eq:xtxttopequation2} is dominant and that it approximates the covariance of the optimal policy. The second term will be bounded by a martingale argument and the third term will be bounded using the hypothesis that $\mathsf{R}_T^\pi \leq C\sqrt{T}$.  To this end, we now introduce the following three events:
\begin{equation}
\begin{aligned}\label{eq:3eventsforsfregret}
    \mathcal{E}_{1} &\triangleq \left\{\exists j : \sum_{t=0}^{T-1}W_{t-j}W_{t-j}^\T \nsucc \Sigma_W- I_{\dx}\opnorm{\Sigma_W} T^{3/4} \right\},\\
    \mathcal{E}_{2} &\triangleq \left\{\exists j : \bigopnorm{\sum_{t=0}^{T-1}\sym\left[ B(U_{t-j}+AX_{t-j}))\right](W_{t-j})^\T} \geq  T^{3/4} \right\},\\
    \mathcal{E}_{3} &\triangleq \left\{\exists j : \bigopnorm{\sum_{t=0}^{T-1}\sym (A+BK)X_{t-1}(B(U_{t-j}-KX_{t-j}))^\T} \geq T^{7/8}\right\}.
\end{aligned}
\end{equation}
Below we provide bounds on each of these failure-events, which we will now combine to arrive at a high probability lower bound on \eqref{eq:xtxttopequation2}.

By combining the bounds \eqref{eq:boundevent1},\eqref{eq:boundevent2} and \eqref{eq:boundevent3} with the choice $m=T^{1/16}$ we find that there exist a polynomial function $\mathsf{poly}$ such that as long
\begin{align*}
    T\geq \mathsf{poly}\left(9^{\dx},\opnorm{B},\opnorm{A},\opnorm{Q^{-1}}\opnorm{R},\opnorm{R^{-1}},\opnorm{B},\opnorm{P},\opnorm{K},\opnorm{\Sigma_W},C \right)
\end{align*}
we have
\begin{align*}
    \mathbf{P}\left(X_tX_t^\T \succeq\sum_{j=0}^{T^{1/16}}(A+BK)^j\Bigg[ \Sigma_W T -I_{\dx}(\opnorm{\Sigma_W}T^{3/4}+T^{3/4}+T^{7/8})\Bigg]((A+BK)^\T)^j  \right) \geq 1/2.
\end{align*}

\paragraph{Bounding $\mathcal{E}_{1}$}
Fix $\eta>0$ and $s\geq 1$. We invoke \citet[Exercise 4.7.3]{vershynin2018} to obtain that
\begin{align*}
    \mathbf{P} \left(\sum_{t=0}^{T-1} W_{t-j}W_{t-j}^\T \nsucc \Sigma_W T -\eta I_{\dx}\opnorm{\Sigma_W} T   \right)\leq 2\exp(-s^2\dx)
\end{align*}
for every $s$ satsifying $T \geq c(s/\eta)^2\dx$ for a universal constant $c>0$. Set $\eta=T^{-1/4}$, then for a second universal positive constant $c'$:
\begin{align}\label{eq:boundevent1}
    \mathbf{P} \left(\sum_{t=0}^{T-1} W_{t-j}W_{t-j}^\T \nsucc \Sigma_W T - I_{\dx}\opnorm{\Sigma_W} T^{3/4}   \right)\leq 2\exp\left(-c'T^{1/4}\right).
\end{align}


\paragraph{Bounding $\mathcal{E}_{2}$}
Fix $\eta=1/4$ and let $(v_1,v_1',\dots,v_N,v_N')$ be an optimal $\eta$-cover of $\mathbb{S}^{\dx-1} \times \mathbb{S}^{\dx-1}$. By Chebyshev's inequality:  
\begin{align*}
    & \mathbf{P}\left(\sum_{t=0}^{T-1}2v_{i}^\T\left[ B(U_{t-j}+AX_{t-j}))\right](W_{t-j})^\T v_{i}'\geq T^{3/4}\right)\\
    &\leq \frac{\E \left(\sum_{t=0}^{T-1}2v_{i}^\T\left[ B(U_{t-j}+AX_{t-j}))\right](W_{t-j})^\T v_{i}'\right)^2}{T^{3/2}}\\
    &\leq \frac{2\sum_{t=0}^{T-1} \opnorm{B}^2 \E \left( \left[ (U_{t-j}+AX_{t-j}))\right]^\T\left[ (U_{t-j}+AX_{t-j}))\right] \right)\tr \Sigma_W }{T^{3/2}}\\
    &\leq \frac{4 \opnorm{B}^2(\opnorm{A}^2\opnorm{Q^{-1}}\vee \opnorm{R^{-1}} ) [V_{T}^\star+R_{T}^\pi] \tr \Sigma_W }{T^{3/2}}\\
    &\leq  \frac{4 \opnorm{B}^2(\opnorm{\opnorm{A}^2Q^{-1}}\vee \opnorm{R^{-1}} ) [\tr(P\Sigma_W)T+C\sqrt{T}] \tr \Sigma_W }{T^{3/2}}\\
    &\leq \frac{4 \opnorm{B}^2(\opnorm{A}^2\opnorm{Q^{-1}}\vee \opnorm{R^{-1}} ) [\tr(P\Sigma_W)+C] \tr \Sigma_W }{T^{1/2}}.
\end{align*}

By \citet[Exercise 4.4.3]{vershynin2018}, we have
\begin{multline*}
    \bigopnorm{\sum_{t=0}^{T-1}\sym\left[ B(U_{t-j}+AX_{t-j}))\right](W_{t-j})^\T} \\ \leq \frac{1}{1-2\eta} \sup_{v_i,v_i'}\left\|\sum_{t=0}^{T-1}2v_i^\T\left[ B(U_{t-j}+AX_{t-j}))\right](W_{t-j})^\T v_i' \right\|_2.
\end{multline*}
Hence by a union bound it follows that (inserting $\eta=1/4$): 
\begin{multline}\label{eq:boundevent2}
    \mathbf{P} \left\{\exists j : \bigopnorm{\sum_{t=0}^{T-1}\sym\left[ B(U_{t-j}+AX_{t-j}))\right](W_{t-j})^\T} \geq  2 T^{3/4} \right\}\\
    \leq\frac{4 m 9^{2\dx} \opnorm{B}^2(\opnorm{A}^2\opnorm{Q^{-1}}\vee \opnorm{R^{-1}} ) [\tr(P\Sigma_W)+C] \tr \Sigma_W }{T^{1/2}}.
 \end{multline}
\paragraph{Bounding $\mathcal{E}_{3}$}
Fix $\eta=1/4$ and let $(v_1,v_1',\dots,v_N,v_N')$ be an optimal $\eta$-cover of $\mathbb{S}^{\dx-1} \times \mathbb{S}^{\dx-1}$. Let $\mathcal{E}_{3,i}$ be the event that 
\begin{align*}
    \sum_{t=0}^{T-1}2v_i^\T (A+BK)X_{t-1}(B(U_{t-j}-KX_{t-j}))^\T v_{i}'
\end{align*}
is nonnegative. By Markov's inequality and Cauchy-Schwarz:
\begin{align*}
    & \mathbf{P}\left( \sum_{t=0}^{T-1}2v_i^\T (A+BK)X_{t-1}(B(U_{t-j}-KX_{t-j}))^\T v_{i}'\geq T^{7/8}\right)\\
    &=\mathbf{P}\left( \sum_{t=0}^{T-1}2v_i^\T (A+BK)X_{t-1}(B(U_{t-j}-KX_{t-j}))^\T v_{i}' \mathbf{1}_{\mathcal{E}_{3,i}}\geq T^{7/8}\right)\\
    &\leq \frac{\E \left(\sum_{t=0}^{T-1}2v_i^\T (A+BK)X_{t-1}(B(U_{t-j}-KX_{t-j}))^\T v_{i}'\mathbf{1}_{\mathcal{E}_{3,i}} \right)}{T^{7/8}}\\
    &= T \frac{\E \left(\frac{1}{T}\sum_{t=0}^{T-1}2v_i^\T (A+BK)X_{t-1}(B(U_{t-j}-KX_{t-j}))^\T v_{i}'\mathbf{1}_{\mathcal{E}_{3,i}} \right)}{T^{7/8}}\\
    &\leq 2T \frac{\sqrt{\E \left(\frac{1}{T}\sum_{t=0}^{T-1}\|(A+BK)X_{t-1}\|_2^2 \right) }\sqrt{\E \left(\frac{1}{T}\sum_{t=0}^{T-1}\|(B(U_{t-j}-KX_{t-j})) \|_2^2 \right) } }{T^{7/8}}\\
    &\leq 2 \frac{\sqrt{ \opnorm{A+BK}^2 \opnorm{Q^{-1}}^2 (V_T^\star+\mathsf{R}_T^\pi) }\sqrt{\opnorm{B}^2\opnorm{(B^\top P B+R)^{-1}} \mathsf{R}_T^\pi } }{T^{7/8}}\\
    &\leq 2 \frac{\sqrt{ \opnorm{A+BK}^2 \opnorm{Q^{-1}}^2 (T \tr P\Sigma_W +C\sqrt{T}) }\sqrt{\opnorm{B}^2\opnorm{(B^\top P B+R)^{-1}} C\sqrt{T} } }{T^{7/8}}\\
    &\leq 2 \frac{\sqrt{ \opnorm{A+BK}^2 \opnorm{Q^{-1}}^2 ( \tr P\Sigma_W +C) }\sqrt{\opnorm{B}^2\opnorm{(B^\top P B+R)^{-1}} C} }{T^{1/8}}.
\end{align*}
Thus by another union bound:
\begin{multline}\label{eq:boundevent3}
    \mathbf{P}\left\{\exists j : \bigopnorm{\sum_{t=0}^{T-1}\sym (A+BK)X_{t-1}(B(U_{t-j}-KX_{t-j}))^\T} \geq 2 T^{7/8}\right\} \ \\
   \leq 2m 9^{2\dx} \frac{\sqrt{ \opnorm{A+BK}^2 \opnorm{Q^{-1}}^2 ( \tr P\Sigma_W +C) }\sqrt{\opnorm{B}^2\opnorm{(B^\top P B+R)^{-1}} C} }{T^{1/8}}.
\end{multline}





\subsection{Proof of Corollary~\ref{statefeedbackcorr}}
We consider the coordinates 
\begin{equation}
\begin{aligned}
\label{eq:corrconsab}
\VEC A(\theta) &= \VEC A-\VEC [ (\VEC^{-1} \theta) K]\\
\VEC B(\theta) &= \VEC B +\theta
\end{aligned}
\end{equation}
By virtue of Proposition~\ref{simchoprop} we know that the instance is $\e$-locally uninformative (for every $\e >0$) with $d_\theta=\dim \mathtt{U} = \dx\du$. By \Cref{thm:sfregretlb} there exists $W_0$ with $\lceil \dx\du/2 \rceil$-many independent columns that satisfy $\spn W_0 \subset \mathtt{U}$.


Using Lemma~\ref{statefeedbackinfocomp} we may choose \begin{align*}
L=\tr(\Sigma^{-1}_w)\left( \sup_{\bar\theta\in B(\theta,\e)} \| \dop_\theta[A(\bar \theta) \:  B(\bar \theta)] \|_\infty^2\right) \|(B^\top P(\theta)B+R)^{-1}\|_{\mathsf{op}}
\end{align*}
with $\e$ arbitrary.  Using (\ref{eq:corrconsab}), we have $\|\dop_\theta[A(\bar \theta) \:  B(\bar \theta)] \|_{\mathsf{op}}^2 \leq 1\vee \| K(\theta)K^\top(\theta)\|_{\mathsf{op}}$. Next, note that
\begin{align*}
 \|(B^\top P(\theta)B+R)^{-1}\|_{\mathsf{op}} = \frac{1}{\sigma_{\min}(B^\top(\theta)  P(\theta)B(\theta)+R)},
\end{align*}
that $\tr \Sigma^{-1}_w \leq \sigma_{\max}(\Sigma^{-1}_w) \dx = \frac{\dx}{\sigma_{\min}(\Sigma_W)}$.  Hence, we may take
\begin{align*}
L \leq \frac{\dx (1\vee \| K(\theta)K^\top(\theta)\|_{\mathsf{op}})}{\sigma_{\min} (\Sigma_W) \times \sigma_{\min} (B^\top(\theta)  P(\theta)B(\theta)+R) }.
\end{align*}


Moreover,
\begin{align*}
\tr\Bigg( [\Sigma^\star_X(\theta) \otimes    (B^\top(\theta) P(\theta)B( \theta)+R)] \left(\dop_\theta\VEC K( \theta) \right)  W_0W_0^\T\left(\dop_\theta \VEC K( \theta) \right)^\top\Bigg)\\
\geq \sigma_{\min} (\Sigma^\star_X(\theta)) \sigma_{\min}\left(B^\top(\theta)  P(\theta)B(\theta)+R\right) \tr 
\Bigg( \left(\dop_\theta\VEC K( \theta) \right) W_0W_0^\T\left(\dop_\theta \VEC K( \theta) \right)^\top\Bigg).
\end{align*}
Moreover, for this parametrization, appealing to Proposition~\ref{simchoprop} and  by virtue of \cref{simchoprop}, we have an explicit expression for $\dop_\theta\VEC K( \theta)   $. Namely, 
\begin{align*}
\dop_\theta\VEC K( \theta) =- \left( (A(\theta)+B(\theta)K(\theta))^\top P(\theta) \right) \otimes \left(B^\top(\theta) P(\theta) B(\theta)+R\right)^{-1} .
\end{align*}
It follows that 
\begin{align*} 
&\tr 
\Bigg( \left(\dop_\theta\VEC K( \theta) \right)  W_0W_0^\T\left(\dop_\theta \VEC K( \theta) \right)^\top\Bigg)\\
&\geq (\dim \mathtt{U}/2)  \frac{\sigma_{\min} (A(\theta)+B(\theta)K(\theta))^2 \sigma_{\min} P^2(\theta) }{\sigma_{\max} \left(B^\top(\theta) P(\theta) B(\theta)+R\right)^{2} }
\end{align*}
which therefore implies
\begin{align*}
&\tr\Bigg( [\Sigma^\star_X(\theta) \otimes    (B^\top(\theta) P(\theta)B( \theta)+R)] \left(\dop_\theta\VEC K( \theta) \right)  W_0W_0^\T\left(\dop_\theta \VEC K( \theta) \right)^\top\Bigg)\\
&
\geq  (\dim \mathtt{U}/2 ) \sigma_{\min} (\Sigma^\star_X(\theta))  \frac{ \sigma_{\min}\left(B^\top(\theta)  P(\theta)B(\theta)+R\right)}{\sigma_{\max} \left(B^\top(\theta) P(\theta) B(\theta)+R\right)^{2} } \sigma_{\min} (A(\theta)+B(\theta)K(\theta))^2 \sigma_{\min} P^2(\theta) .
\end{align*}
Combining the above facts and substituting into (\ref{eq:asymptoticlb}) yields the desired result. \hfill $\blacksquare$

\subsection{Proof of \Cref{statefeedbackinfocomp}}
\label{sec:proof:statefeedbackinfocomp}
Fix $\theta'\in B(\theta,\e)$ and let the columns of $V_0$ span the information singular subspace $\mathtt{U}$. We now introduce a quadratic potential, $f:\mathbb{R}^{T(\dx+\du)}\to \mathbb{R}$, in terms of the dummy variables $\eta_j=(\eta_j^1,\eta_j^2) \in \mathbb{R}^{\dx+\du}$ as 
\begin{align}
\label{eq:thepotential}
f(\eta_{0:T-1}) = \tr \left[V_0^\T\left(\sum_{j=1}^{T-1}  \left( \dop_\theta[A(\theta') \:  B(\theta')]\right)^\T ( \eta_{j-1} \eta_{j-1}^\T \otimes \Sigma_{W}^{-1}(\theta)) \left( \dop_\theta[A(\theta') \:  B(\theta')]\right) \right) V_0 \right].
\end{align}
Observe that $\E_{\theta'}^\pi f(Z_{0:T-1}) =  \tr V_0^\T \I(\pi;\theta',T) V_0$. Our next observation is that the restriction of $f$ to the subspace $\eta^2_j = K(\theta)\eta^1_j, \forall j$ is identically zero by uniformativeness and invoking \Cref{prop:charpropsf} (recall that the columns of $V_0$ span $\mathtt{U}$).

Since the linear manifold $F_0 =\{\eta^2_j = K(\theta)\eta^1_j, \forall j\}\subset \mathbb{R}^{ T (\dx+\du)}$ is a global minimum for $f$, we may, for any fixed choice of $\eta^1_j,0=1,\dots,T-1$, Taylor-expand $f$ around such a point with coordinate $\eta^1$ fixed, to obtain

\begin{align*}
f(\eta_{0:T-1}) \leq \frac{1}{2} \opnorm{\nabla^2_{\eta^{2}_{0:T-1}} f}  \left \|(\eta^2_j-K(\theta)\eta^1_j)_{j=0}^{T-1} \right\|_2.
\end{align*}
where we have used the fact that $f$ is convex quadratic function with minimum $0$, attained at all points in $F_0$, so that its taylor-expansion around such a point is just a quadratic form. 

By introducing a factor $I_{\du} = (B^\T P(\theta)B+R)^{-1}(B^\T P(\theta)B+R)$ we obtain
\begin{align*}
f(\eta_{0:T-1})& \leq\frac{1}{2} \opnorm{(B^\T P(\theta)B+R)^{-1}} \| \nabla^2_{\eta^{2}_{0:T-1}} f\|_{\mathsf{op}}\\
&\times \sum_{t=0}^{T-1}  (\eta^2_j-K(\theta)\eta_j^1)^\T (B^\T P(\theta)B+R) (\eta_j^2-K(\theta)\eta_j^1)
\end{align*}
In particular, by taking expectations, we have that
\begin{align*}
\tr V_0^\T \I(\pi;\theta',T) V_0 =\frac{1}{2} \E_{\theta'}^\pi f(Z_{0:T-1})  \leq  \opnorm{(B^\T P(\theta)B+R)^{-1}} \opnorm{ \nabla^2_{\eta^{2}_{0:T-1}} f} \mathsf{R}_T^\pi(\theta)
\end{align*}
Since
\begin{align*}
\opnorm{\nabla^2_{\eta^{2}_{0:T-1}} f} \leq \opnorm{ \dop_\theta[A(\theta') \:  B(\theta')] \|}^2 \tr ( \Sigma_W^{-1})
\end{align*}
we have for any $\theta'\in B(\theta,\e)$
\begin{align*}
\tr V_0^\T \I(\pi;\theta',T) V_0 \leq \tr ( \Sigma_W^{-1}) \opnorm{\dop_\theta[A( \theta') \:  B(\theta')] }^2\opnorm{(B^\T P(\theta)B+R)^{-1}} \mathsf{R}_T^\pi(\theta)
\end{align*}
and the result follows.  \hfill $\blacksquare$


